SemEval-2021 Task 11: NLPContributionGraph -- Structuring Scholarly NLP Contributions for a Research Knowledge Graph

There is currently a gap between the natural language expression of scholarly publications and their structured semantic content modeling to enable intelligent content search. With the volume of research growing exponentially every year, a search feature operating over semantically structured content is compelling. The SemEval-2021 Shared Task NLPContributionGraph (a.k.a. 'the NCG task') tasks participants to develop automated systems that structure contributions from NLP scholarly articles in the English language. Being the first-of-its-kind in the SemEval series, the task released structured data from NLP scholarly articles at three levels of information granularity, i.e. at sentence-level, phrase-level, and phrases organized as triples toward Knowledge Graph (KG) building. The sentence-level annotations comprised the few sentences about the article's contribution. The phrase-level annotations were scientific term and predicate phrases from the contribution sentences. Finally, the triples constituted the research overview KG. For the Shared Task, participating systems were then expected to automatically classify contribution sentences, extract scientific terms and relations from the sentences, and organize them as KG triples. Overall, the task drew a strong participation demographic of seven teams and 27 participants. The best end-to-end task system classified contribution sentences at 57.27% F1, phrases at 46.41% F1, and triples at 22.28% F1. While the absolute performance to generate triples remains low, in the conclusion of this article, the difficulty of producing such data and as a consequence of modeling it is highlighted.

==> old-text-system-descriptions.tex <==
\paragraph{YNU-HPCC} This system by~\citeauthor{ynu-hpcc} \citeyearpar{ynu-hpcc} is unique as a BERT out-of-the-box model. \textit{Contribution sentences.} They employed BERT as a binary classifier to identify the contribution sentences from all sentences in an article. \textit{Scientific terms and relations.} They used a pre-trained BERT model for sequence labeling of each token, obtaining embeddings for each token in the sequence, with softmax and argmax top layers which were shared across all tokens. \textit{Triples.} To form triples they applied three binary BERT classifiers to the entities extracted to classify them into subject, predicate, or object roles in triples. They also used a BERT-based classifier to classify sentences by the 12 IUs and the triples were accordingly organized by the IU class assigned to its sentence. This system was not evaluated for end-to-end pipeline testing.

\paragraph{Duluth} Unique about the system by \citeauthor{duluth} \citeyearpar{duluth} was the use of a maximum entropy Markov model (MEMM) to address one of the tasks thereby offering novel insights. \textit{Contribution sentences.} This task was formulated as a 13 multi-class classification. In experiments with logistic regression, decision trees, and a finetuned BERT model variant called deBERTa~\cite{he2020deberta}, deBERTa significantly outperformed the rest. The approach is interesting since it did not downsample the majority non-contribution sentences class during training, and thus it reports a BERT model variant result for multi-class classification trained on an imbalanced class distribution. \textit{Scientific terms and relations.} A maximum entropy Markov model (MEMM) was applied to indicate likely scientific entities. They employed a dependency parser to extract noun phrases and the relation between them from contribution sentences. \textit{Triples.} A dependency parse was then found for each sentence and its entities which were then used to extract (subject,predicate,object) triples. The overall end-to-end pipelined system score achieved by this system is 28.38\%.

\paragraph{INNOVATORS} This system by \citeauthor{innovators} \citeyearpar{innovators} uniquely employ an unsupervized dependency parsing scheme for phrase extraction. \textit{Contribution sentences}. They establish a threshold computed based on cumulative contributing sentence bigram scores as a filter criteria to reduce the number of non-contributing sentences. The candidate sentences are fed into a BERT-based classifier wherein each instances is a set of 10 sentences with additional sentences as context features to the model. \textit{Scientific terms and relations.} Differing from all existing teams, they use an unsupervized rule-based dependency parsing system for phrase extraction. \textit{Triples.} A CNN-based architecture for classifying sentences to 12 information units followed by a set of rules to generate triples. Their overall end-to-end system score of 32.05\%.

\paragraph{ECNUICA} The \citeauthor{ecnuica} \citeyearpar{ecnuica} system ranked fourth within the official task timeline for the End-to-end Evaluation. Unique to their model is an ensemble of three pretrained transformer models, viz. RoBERTa~\cite{liu2019roberta}, SciBERT~\cite{Beltagy2019SciBERT}, and BERT~\cite{devlin2019bert} as a classifier. Further, to compensate for imbalanced data distribution within NLP subdomains, they feedback into the learning system automatically classified data as silver-labeled training data. \textit{Contribution Sentences.} They formulate this as a multi-class classification task with the twelve IU classes and an additional non-contribution class for sentence classification. They employ an ensemble classifier comprising three BERT variants. In a first pass, the BERT variants are independently trained on gold data. In a second pass, silver-labeled classified sentences are obtained by classifying unannotated sentences using the BERT models and in particular only those sentences classified unanimously as the same class. Finally, in a third pass, the gold and silver labeled data are combined to train a final ensemble sentence classifier. The features to BERT models are the original sentence, contextual information as previous and next sentence to the original sentence, and a sub-title of the paragraph with the separator token ([SEP]) in between.
\textit{Scientific terms and relations.} They extract entities using RoBERTa with a CRF layer and a BIO sequence labeling scheme. \textit{Triples.} They form candidate triples as sequences of extracted phrases from the sentences. Additionally, each triple predicate is replaced by a set of predefined predicates to be used when a predicate cannot be directly extracted from the sentence text. Then a SciBERT-based binary classifier is used to classify the true triples from the candidates. Finally, triples with inter-sentence arguments are formed directly from the extracted data, i.e. if a sentence has only one extracted entity, without machine learning. Their overall end-to-end system score was 33.35\%.

\paragraph{KnowGraph@IITK} This system by \citeauthor{knowgraph-iitk} \citeyearpar{knowgraph-iitk} ranked third within the official task timeline for the End-to-end Evaluation. Crucially, this system adopts the SciBERT model~\cite{Beltagy2019SciBERT}, i.e. the BERT transformer model~\cite{devlin2019bert} pretrained on scientific articles from biomedical and computer sciences domain thus making SciBERT better suited to the NLPContributionGraph corpus of scholarly articles. \textit{Contribution Sentences.} The used the standard SciBERT + BiLSTM architecture as the classifier. \textit{Scientific terms and relations.} They use the same classification architecture as the first task except they additionally append a Conditional Random Field (CRF) layer for sequence labeling based on the BILUO scheme. \textit{Triples.} Based on dataset observations, they aptly identify four information units, \textsc{ResearchProblem}, \textsc{Code}, \textsc{AblationAnalysis}, and \textsc{Baselines}, as being addressable by a heuristics-based approach. For the remaining eight IUs, they formulate a 8-class classification task, where they employ SciBert-based multi-class classification for the triples. Their overall end-to-end system score was 37.83\%.


\paragraph{ITNLP} The top-performing system within the official task timeline for the End-to-end Evaluation Phase was the ITNLP system by \citeauthor{itnlp} \citeyearpar{itnlp}. The system is composed of three BERT-based models addressing the separate aspects of the \textsc{NLPContributionGraph} extraction task, i.e. sentences, entities, and triples, respectively. Crucial to the system was leveraging sampling and adversarial training strategies to boost BERT performances thereby producing the high scores. \textit{Contribution sentences.} They adopted the standard BERT classifier with additional features of the sentence as context and paragraph heading. Further, they undersampled the negative training instances, i.e. the non-contribution sentences, to prevent classifier overfitting on this majority class. \textit{Scientific terms and relations.} They employed the standard BERT-based model however in a sequence labeling setting. They trained ten different models by ten-fold cross-validation and used a voting count threshold scheme to extract the final set of entities. \textit{Triples.} Entities in sequence were joined as triples which were then classified by BERT. They also employ the sentence context as a feature. The negative triples were generated as follows: by artificially generating them using random replacement of one of the arguments of the true triples with a false argument and by random selection of triples where no argument is a valid pair of another. For each group they apply undersampling. Finally, each of the tasks obtained boosted performances since they were trained with the Friendly Adversarial Training strategy~\cite{zhang2020attacks}. Their overall end-to-end system score including all three aspects was 47.03\%.

\paragraph{UIUC\_BioNLP} This overall top-performing system by \citeauthor{uiuc-bionlp} \citeyearpar{uiuc-bionlp} adopted an overarching strategy that combined a cascade of state-of-the-art BERT-based classification and sequence labeling models with rule-based methods. \textit{Contribution sentences.} Their BERT-based sentence classifier was fitted with additional features that modeled the sentence selection criteria of the dataset design - that contribution sentences were commonly selected from the title, abstract and first few lines of each section, rather the main section content or from a section about Related Work. The additional features in their BERT model handled such sentence features w.r.t. its context in the article - specifically, its closest preceding topmost and innermost headers and its position in the document. \textit{Scientific terms and relations.} They modeled this as a standard NER task with a BIO scheme with separate labels for predicates and terms leveraging a BERT model with a CRF layer. \textit{Triples.} They categorized triples data into six types based on dataset design and addressed each type with a specifically trained BERT classifier. The six categories were based on whether the subject or object phrase was modeled from the sentence itself or was the dummy node or the IU name; and whether predicates were annotated from the sentence itself or was the generic predicate ``has.'' Finally, the system integrates rules in place of machine learning to address the less diverse triples information types that can be easily addressed by few human observations of the data. Their overall end-to-end system score including all three aspects was 38.28\% within the task deadline and 49.72\% a day later after fixing phrase component offset errors.\footnote{Per the task timeline, i.e. within the Phase 1 end-to-end system evaluation, the team achieved 38.28\% F-score within the task deadline due to an error in their submission offsets for phrases. Thus, they are officially second ranked after the ITNLP team within the Shared Task timeline for Phase 1.}





